Cooperative Localisation of a GPS-Denied UAV using Direction of Arrival Measurements

A GPS-denied UAV (Agent B) is localised through INS alignment with the aid of a nearby GPS-equipped UAV (Agent A), which broadcasts its position at several time instants. Agent B measures the signals' direction of arrival with respect to Agent B's inertial navigation frame. Semidefinite programming and the Orthogonal Procrustes algorithm are employed, and accuracy is improved through maximum likelihood estimation. The method is validated using flight data and simulations. A three-agent extension is explored.

==> parts/next.tex <==
\subsection{Scope for further refinement}

The estimation $\overline{R}$ has the potential to be further refined though the use of maximum likelihood estimation. This process consists of minimising the cumulative error between expected and measured bearing angles for a given estimation of $\bm{R_A^B}$ and $\bm{T_A^B}$. This is achieved by evaluating the gradient over the cost function of cumulative error, and running a gradient descent algorithm using partial derivatives corresponding to the 6 degrees of freedom in the problem.
